Generic Reduction-Based Interpreters (Extended Version)

Reduction-based interpreters are traditionally defined in terms of a one-step reduction function which systematically decomposes a term into a potential redex and context, contracts the redex, and recomposes it to construct the new term to be further reduced. While implementing such interpreters follows a systematic recipe, they often require interpreter engineers to write a substantial amount of code -- much of it boilerplate. In this paper, we apply well-known techniques from generic programming to reduce boilerplate code in reduction-based interpreters.

==> latexmkrc <==
$out_dir = "build";

$tex_src .= "\\input{%S}";

$bibtex_use = 2;

$ENV{'BIBINPUTS'}='../tex';

$pdf_mode = 1;
$pdflatex = "texfot xelatex %O -interaction=nonstopmode -synctex=1 -shell-escape \"$tex_src\"";


==> macros/color.tex <==
\definecolor{gray_ulisses}{gray}{0.55}
\definecolor{castanho_ulisses}{rgb}{0.71,0.33,0.14}
\definecolor{preto_ulisses}{rgb}{0.41,0.20,0.04}
\definecolor{green_ulises}{rgb}{0.2,0.75,0}
\definecolor{picolor}{rgb}{0.4,0.1,0.4}
\definecolor{starcolor}{rgb}{0.7, 0.35, 0}
\definecolor{opcolor}{rgb}{0 , 0.3 , 0.3}

==> macros/general.tex <==
\newcommand{\Type}{{\color{starcolor}\star}}

% Homogeneous data type composition
\newcommand{\CompOp}{\sqcup}
\newcommand{\Comp}[2]{{#1} \CompOp{} {#2}}

% Homogeneous data type intersection
\newcommand{\InterOp}{\sqcap}
\newcommand{\Inter}[2]{{#1} \InterOp{} {#2}}

% Homogeneous data type difference
\newcommand{\DiffOp}{\ /\ }
\newcommand{\Diff}[2]{{#1} \DiffOp {#2}}

% Homogeneous data type union
\newcommand{\UnionOp}{\cup}
\newcommand{\Union}[2]{{#1} \UnionOp {#2}}

% Heterogeneous data type composition
\newcommand{\ParOp}{\dot \sqcup}
\newcommand{\Par}[2]{{#1}\ \ParOp\ {#2}}

% Heterogeneous data type intersection
\newcommand{\HInterOp}{\dot \sqcap}
\newcommand{\HInter}[2]{{#1}\ \HInterOp\ {#2}}

% Heterogeneous data type difference 
\newcommand{\HDiffOp}{\mathbin{\!/\mkern-5mu/\!}}
\newcommand{\HDiff}[2]{{#1}\ \HDiffOp\ {#2}}

% Heterogeneous data type union
\newcommand{\HUnionOp}{\dot \cup}
\newcommand{\HUnion}[2]{{#1}\ \HUnionOp\ {#2}}

% projections
\newcommand{\proj}[2]{\boldsymbol{\color{picolor}\pi_{#1}}\ #2}

\newcommand{\ParRel}[3]{\Par{#1}{#2} \equiv #3}

\newcommand{\SubOp}{\sqsubseteq}
\newcommand{\Sub}[2]{#1 \SubOp #2}

\newcommand{\SubPOp}{\dot \sqsubseteq}
\newcommand{\SubP}[2]{#1\ \SubPOp\ #2}

\renewcommand{\Join}[2]{{#1} \JoinOp{} {#2}}
\newcommand{\JoinRel}[3]{\Comp{#1}{#2} \equiv #3}

\newcommand{\Widen}[2]{{#1} \bigtriangledown {#2}}
\newcommand{\InjOp}{\mathit{inj}}
\newcommand{\Inj}[1]{\InjOp\ #1}
\newcommand{\MonoOp}{\mathit{Mono}}
\newcommand{\Mono}[2]{\MonoOp\ {#1}\ {#2}}
\newcommand{\DisjOp}{\mathit{Disjoint}}
\newcommand{\Disj}[2]{\DisjOp\ {#1}\ {#2}}
\newcommand{\Member}[2]{{#1} \in {#2}}
\newcommand{\MemberI}[2]{{#1} \in^{\mathsf{i}} {#2}}
\newcommand{\TOW}{\rightarrowtail}
\newcommand{\WidenCD}[2]{{#1} \mathop{\blacktriangledown^{\mathsf{c}}} {#2}}
\newcommand{\WidenFN}[2]{{#1} \mathop{\blacktriangledown^{\mathsf{f}}} {#2}}
\newcommand{\ComposeOp}{\oplus}
%% \newcommand{\Compose}[2]{{#1} \ComposeOp{} {#2}}
%% \newcommand{\ComposeFragOp}{\mathop{\ComposeOp{}^{\mathsf{F}}}}
%% \newcommand{\ComposeFrag}[2]{{#1} \ComposeFragOp{} {#2}}

\newcommand{\Denote}[1]{{\color{opcolor}\llbracket {#1} \rrbracket}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../document"
%%% End:


==> macros/todo.tex <==
% depends on toggle draft being set

\RequirePackage{geometry}
\iftoggle{draft}
{
  \newgeometry{twoside=true,
     includeheadfoot, head=13pt, foot=2pc,
     paperwidth=\dimexpr 6.75in + 6cm \relax, paperheight=10in,
     top=58pt, bottom=44pt, inner=46pt, outer=\dimexpr 46pt + 5cm\relax,
     marginparwidth=6cm,heightrounded
  }
  % \paperwidth=\dimexpr\paperwidth+6cm\relax
  % \evensidemargin=\dimexpr\evensidemargin+5cm\relax
  % \marginparwidth=\dimexpr\marginparwidth+5cm\relax
  % \marginparsep=1cm
}{}
\RequirePackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\RequirePackage{xcolor}
\newcommand{\comm}[3]{%
  \iftoggle{draft}%
    {\todo[linecolor=#1,backgroundcolor=#1!25,bordercolor=#1]{[#2] #3}}%
    {}}
\newcommand{\TODO}[1]{\comm{red}{TODO}{#1}}
\newcommand{\ITODO}[1]{{\color{red} #1}}
\newcommand{\aj}[1]{\comm{cyan}{AJ}{#1}}
\newcommand{\cbp}[1]{\comm{green}{CBP}{#1}}
\newcommand{\ev}[1]{\comm{blue}{EV}{#1}}
\newcommand{\pe}[1]{\comm{white}{PM}{#1}}
\newcommand{\cas}[1]{\comm{purple}{CAS}{#1}}
\newcommand{\resolved}[2][]{\comm{gray}{#1}{\sout{#2}}}
\newcommand{\wontfix}[3][]{\comm{gray}{#1}{WONTFIX: \sout{#2} #3}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../document"
%%% End:


==> sections/06-examples.tex <==
\begin{code}[hide]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{sections.06-examples}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\end{code}

\section{Examples of Reduction Semantics}


